DLPNO-MP2 for Periodic Systems using Megacell Embedding

We present a domain-based local pair natural orbital M{\o}ller--Plesset second order perturbation theory (DLPNO-MP2) for periodic systems, working within an LCAO formalism within the Tubromole program package. This approach, Megacell-DLPNO-MP2, embeds a supercell correlation treatment within a megacell and does not involve periodic image summation for the Coulomb integrals. Working in a basis of well-localised Wannier functions, periodicity is instead imposed through rigorous translational symmetry of Hamiltonian integrals and wavefunction parameters. The accuracy of the method is validated through comparison with a complementary periodic DLPNO-MP2 method that employs Born--von K{\'a}rm{\'a}n boundary conditions, described in paper I of this series. The PNO approximations are shown to be equivalent in the two approaches and entirely consistent with molecular DLPNO-MP2 calculations. The Megacell-DLPNO-MP2 method displays sub-linear scaling with respect to supercell size at the asymptotic limit and example calculations are presented with up to 15000 basis functions in the correlation treatment.

==> data.tex <==
\section*{Supporting Information}
\label{si}

\begin{table*}[tbp]
    \begin{ruledtabular}
    \centering
    \caption{1D  C$_{2}$H$_{2}$ with pob-TZVP-rev2 basis, universal jbas and def2-TZVP cbas. PNO threshold set to $10^{-7}$. All energies (per unit cell) are in Hartree. nfroz=2. Analysis of effect of Wannier extension scheme, compared to HF calculations calculated using the k-grid of the megacell. \textcolor{red}{Old data with at lower PM optimisation threshold, old tolint, and no scftol.}}
    \begin{tabular}{r c c c c c}
    \multicolumn{1}{c}{HF $\mathbf{k}$-mesh} & \multicolumn{1}{c}{$E_\mathrm{HF}$} & \multicolumn{1}{c}{Megacell size} & \multicolumn{1}{c}{Supercell size} &
    \multicolumn{1}{c}{$E_\mathbf{MP2}$} \\
    \hline
      9 & -76.89458 &  9 &  5 & -0.27500 &     \\
     13 & -76.89448 & 13 &  7 & -0.27558 &     \\
     17 & -76.89447 & 17 &  9 & -0.27569 &     \\
     21 & -76.89447 & 21 & 11 & -0.27571 &     \\
     25 & -76.89447 & 25 & 13 & -0.27571 &     \\
     29 & -76.89447 & 29 & 15 & -0.27572 &     \\
     33 & -76.89447 & 33 & 17 & -0.27571 &     \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
      9 &  & 13 &  7 & -0.27565      \\
      9 &  & 17 &  9 & -0.27578      \\
      9 &  & 21 & 11 & -0.27580      \\
      9 &  & 25 & 13 & -0.27580      \\
      9 &  & 29 & 15 & -0.27580      \\
      9 &  & 33 & 17 & -0.27580      \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
     13 &  & 33 & 17 & -0.27572      \\
     17 &  & 33 & 17 & -0.27572      \\
     21 &  & 33 & 17 & -0.27571      \\
     25 &  & 33 & 17 & -0.27571      \\
     29 &  & 33 & 17 & -0.27572      \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
     13 &  & 17 & 9 & -0.27570      \\
     13 &  & 21 & 11 & -0.27572      \\
     13 &  & 25 & 13 & -0.27572      \\
     13 &  & 29 & 15 & -0.27573      \\
    \end{tabular}
    \end{ruledtabular}
\end{table*}

\begin{table*}[tbp]
    \begin{ruledtabular}
    \centering
    \caption{1D  C$_{2}$H$_{2}$ with pob-TZVP-rev2 basis, universal jbas and def2-TZVP cbas. PNO threshold set to $10^{-7}$. All energies (per unit cell) are in Hartree. nfroz=2. PM gradient norm threshold: $10^{-7}$. scftol set to $10^{-12}$. Analysis of effect of Wannier extension scheme, compared to HF calculations calculated using the k-grid of the megacell}
    \begin{tabular}{r c c c c c}
    \multicolumn{1}{c}{HF $\mathbf{k}$-mesh} & \multicolumn{1}{c}{$E_\mathrm{HF}$} & \multicolumn{1}{c}{Megacell size} & \multicolumn{1}{c}{Supercell size} &
    \multicolumn{1}{c}{$E_\mathbf{MP2}$} \\
    \hline
      9 & -76.89458 &  9 &  5 & -0.27499 &     \\
     13 & -76.89448 & 13 &  7 & -0.27556 &     \\
     17 & -76.89447 & 17 &  9 & -0.27568&     \\
     21 & -76.89447 & 21 & 11 & -0.27570 &     \\
     25 & -76.89447 & 25 & 13 & -0.27570 &     \\
     29 & -76.89447 & 29 & 15 & -0.27570 &     \\
     33 & -76.89447 & 33 & 17 & -0.27571 &     \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
      9 &  & 13 &  7 & -0.27565      \\
      9 &  & 17 &  9 & -0.27578      \\
      9 &  & 21 & 11 & -0.27580      \\
      9 &  & 25 & 13 & -0.27580      \\
      9 &  & 29 & 15 & -0.27580      \\
      9 &  & 33 & 17 & -0.27580      \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
     13 &  & 17 & 9 & -0.27570      \\
     13 &  & 21 & 11 & -0.27572      \\
     13 &  & 25 & 13 & -0.27573      \\
     13 &  & 29 & 15 & -0.27572      \\
     13 &  & 33 & 17 & -0.27572      \\
    \end{tabular}
    \end{ruledtabular}
\end{table*}

\begin{table*}[tbp]
    \begin{ruledtabular}
    \centering
    \caption{Same as above but PNO threshold at $10^{-8}$}
    \begin{tabular}{r c c c c c}
    \multicolumn{1}{c}{HF $\mathbf{k}$-mesh} & \multicolumn{1}{c}{$E_\mathrm{HF}$} & \multicolumn{1}{c}{Megacell size} & \multicolumn{1}{c}{Supercell size} &
    \multicolumn{1}{c}{$E_\mathbf{MP2}$} \\
    \hline
      9 & -76.89458 &  9 &  5 & -0.27513 &     \\
     13 & -76.89448 & 13 &  7 & -0.27571 &     \\
     17 & -76.89447 & 17 &  9 & -0.27584 &     \\
     21 & -76.89447 & 21 & 11 & -0.27586 &     \\
     25 & -76.89447 & 25 & 13 & -0.27588 &     \\
     29 & -76.89447 & 29 & 15 & -0.27587 &     \\
     33 & -76.89447 & 33 & 17 & -0.27588 &     \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
      9 &  & 13 &  7 & -0.27580      \\
      9 &  & 17 &  9 & -0.27593      \\
      9 &  & 21 & 11 & -0.27596      \\
      9 &  & 25 & 13 & -0.27596      \\
      9 &  & 29 & 15 & -0.27596      \\
      9 &  & 33 & 17 & -0.27596      \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
     13 &  & 17 &  9 & -0.27586      \\
     13 &  & 21 & 11 & -0.27589      \\
     13 &  & 25 & 13 & -0.27590      \\
     13 &  & 29 & 15 & -0.27590      \\
     13 &  & 33 & 17 & -0.27590      \\
    \end{tabular}
    \end{ruledtabular}
\end{table*}


\begin{table*}[tbp]
    \begin{ruledtabular}
    \centering
    \caption{2D  BN with pob-TZVP basis, universal jbas and def2-TZVP cbas. All energies (per unit cell) are in Hartree. nfroz=2. scftol=1d-12. HF, MP2 energies. CPU times on a single thread. Denis' most converged value was -0.21874. \textcolor{red}{pdens and 3idx integral generation scales to a constant value, BUT pno-paos and num3idxovl have approximately quadratic or sub-quadratic scaling. For tolpno7, other subroutines which aren't time profiled also begin to grow in contribution to CPU time- the sum of the time profiles is only 60-80\% compared to 90\% at lower k grids/ higher tolpnos.}}
    \begin{tabular}{c c c c c c c c c c c c}
    \multicolumn{1}{c}{tolpno} & \multicolumn{1}{c}{HF $\mathbf{k}$ grid} & \multicolumn{1}{c}{Supercell size} & \multicolumn{1}{c}{$E_\mathbf{HF}$} & 
    \multicolumn{1}{c}{$E_\mathbf{MP2}$} & \multicolumn{1}{c}{CPU total (s)} & \multicolumn{1}{c}{3idx} & \multicolumn{1}{c}{pairscreen} & 
    \multicolumn{1}{c}{prepnos} &\multicolumn{1}{c}{pdens} & \multicolumn{1}{c}{paos} &\multicolumn{1}{c}{num3}\\
    \hline
      6 & 9 & 5 & -79.29075 & -0.21750    \\
      & 13 & 7 & -79.29075 & -0.21767    \\
      & 17 & 9 & -79.29075 &-0.21772     \\
      & 21 & 11 & -79.29075 &-0.21773     \\
      & 25 & 13 & -79.29075 & -0.21774    \\

    \hline
    \multicolumn{5}{c}{} \\
    \hline
      7 & 9 & 5 & &-0.21811 & 1084 & 228 & 20 & 13 & 564& 3& 57       \\
      & 13 & 7 & &-0.21832 &2105&	440&	39	&42 &956 &23	&155   \\
      & 17 & 9 & &-0.21836&2974&	360&	55&	113& 1348& 108	&321     \\
      & 21 & 11 && -0.21837 & 3852&	353&	77&	246 &873& 372 &571    \\
      & 25 & 13 && -0.21838 &7501&	369&	97	&475& 1425& 1034 &933    \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
      8 & 9 & 5 & &-0.21832 &2521&	259	&52	&18&	1811&	3&	56   \\
      & 13 & 7 &  &-0.21856 &5761&	859	&148&	59	&3445	&24	&154  \\
      & 17 & 9 &   &-0.21860&7242&	1054&	224&	139	&3769	&108	&327 \\
      & 21 & 11 &  & -0.21861  &8812&	926&	266&	294&	4017&	252&	558 \\
      & 25 & 13  &&-0.21862  &11950	&934&	312	&552	&4084&	695&	900  \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
      9 & 9 & 5 &  & -0.21839&4942&	270	&84&	26 &4037&$<$5& $<$5     \\
      & 13 & 7 & & -0.21866&15431&	1082&	326	&88&11877& 18& 185   \\
      & 17 & 9 & & -0.21870 & 22629	&2301	&608&	201& 14970& 18& 158    \\
      & 21 & 11 & & -0.21872 &28285	&3155	&859&	388  & 16442 & 251 & 560 \\
      & 25 & 13 & &-0.21872  & 34458&	3218&	1034	&714 & 18544 & 687 & 904 \\
    \end{tabular}
    \end{ruledtabular}
\end{table*}

\begin{table*}[tbp]
    \begin{ruledtabular}
    \centering
    \caption{Table for all 3D data. pob-TZVP orbital basis. def2-TZVP cbas. universal jbas. tolint fixed at 5d-6 (or greater). pmoptim threshold 1d-7. Denis' limit value for MgO and LiH were -0.03105 and -0.19931, respectively.}
    \begin{tabular}{c c c c c }
    \multicolumn{1}{c}{PNO threshold} &
    \multicolumn{1}{c}{$E_\mathbf{MP2}$} &
    \multicolumn{1}{c}{Supercell size} & \multicolumn{1}{c}{$E_\mathbf{HF}$} & 
    \multicolumn{1}{c}{nbf in supercell} \\
    \hline
    MgO & ncore=6 \\
    \hline
      6 & -0.19904 & 7,7,7 & -274.68455 & 12691   \\
      7 & -0.19919 &  &  &    \\
      8 & -0.19928 &  & &    \\
      \\
      6 & -0.19868 & 5,5,5 & -274.68455 & 4625   \\
      7 & -0.19897 &  &  &    \\
      8 & -0.19908 &  & &    \\
      \\
      6 & -0.19747 & 5,5,5 & -274.68452 & 999   \\
      7 & -0.19765 &  &  &    \\
      8 & -0.19774 &  & &    \\
    \hline
    LiH & ncore=1 \\
    \hline
      6 & -0.03083 & 7,7,7 & -8.06059 & 4459   \\
      7 & -0.03091 &  &  &    \\
      8 & -0.03096 &  & &    \\
      9 & -0.03098 &  & &    \\
    \hline
    Si & ncore=10 \\
    \hline
      6 & -0.17394 & 5,5,5 & -577.84720 & 5500   \\
      7 & -0.17637 &  &  &    \\
      8 & -0.17703 &  & &    \\
      \\
      6 &-0.16401  & 3,3,3 & -577.84603 & 1188   \\
      7 & -0.16507 &  &  &    \\
      8 &-0.16542  &  & &    \\
    \hline
    C & ncore=2 \\
    \hline
      5 & -0.26921 &   &  &    \\
      6 & -0.27480 & 5,5,5 & -75.77007 & 4500   \\
      7 & -0.27668 &   &  &    \\
      8 &  &  & &    \\
    \hline
    Ice- Ih & ncore=4 \\
    \hline
      5 & -0.74310  &  &  &    \\
      6 & -0.74620 & 5,5,5 & -304.26198  & 15000   \\
      7 & -0.74738  &  &  &    \\
      8 & -0.74781 &  & &    \\
      \\
      6 & -0.74541 & 3,3,3 & -304.26198 & 3240   \\
      7 & -0.74677 &  &  &    \\
      8 & -0.74727 &  & &    \\
    \end{tabular}
    \end{ruledtabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

